OmChat: A Recipe to Train Multimodal Language Models with Strong Long Context and Video Understanding

We introduce OmChat, a model designed to excel in handling long contexts and video understanding tasks. OmChat's new architecture standardizes how different visual inputs are processed, making it more efficient and adaptable. It uses a dynamic vision encoding process to effectively handle images of various resolutions, capturing fine details across a range of image qualities. OmChat utilizes an active progressive multimodal pretraining strategy, which gradually increases the model's capacity for long contexts and enhances its overall abilities. By selecting high-quality data during training, OmChat learns from the most relevant and informative data points. With support for a context length of up to 512K, OmChat demonstrates promising performance in tasks involving multiple images and videos, outperforming most open-source models in these benchmarks. Additionally, OmChat proposes a prompting strategy for unifying complex multimodal inputs including single image text, multi-image text and videos, and achieving competitive performance on single-image benchmarks. To further evaluate the model's capabilities, we proposed a benchmark dataset named Temporal Visual Needle in a Haystack. This dataset assesses OmChat's ability to comprehend temporal visual details within long videos. Our analysis highlights several key factors contributing to OmChat's success: support for any-aspect high image resolution, the active progressive pretraining strategy, and high-quality supervised fine-tuning datasets. This report provides a detailed overview of OmChat's capabilities and the strategies that enhance its performance in visual understanding.

==> backup.tex <==
\begin{longtable}[ht]{@{}ccc@{}}
\caption{\textbf{Summary of datasets used in the multimodal pretraining stage}} 
\label{tab: Summary of pretraining stage} \\
\toprule
Category                   & Dataset                          & Ratio/\% \\ \midrule
\endfirsthead
\caption[]{\textbf{Summary of datasets used in the multimodal pretraining stage (Continued)}} \\
\toprule
Category                   & Dataset                             & Ratio/\% \\ \midrule
\endhead
\bottomrule
\endlastfoot
Image interleaved with text & \begin{tabular}[c]{@{}c@{}}MMC4-Core \citep{zhu2024multimodal}\\
                                                         In-house interleaved data\end{tabular}              & 35.6     \\ \midrule
OCR                         & \begin{tabular}[c]{@{}c@{}}CTW \citep{yuan2019large}\\
                                                         LSVT \citep{sun2019chinese}\\
                                                         ReCTS \citep{yao2012detecting}\\
                                                         ICDAR2019-ArT \citep{chng2019icdar2019}\\
                                                         pdfa-eng-wds \citep{pixparse2024}\end{tabular}                                                                                                                                                          & 18.3     \\ \midrule
Video                       & \begin{tabular}[c]{@{}c@{}}InternVideo \citep{wang2022internvideo}\\
                                                         ActivityNet \citep{caba2015activitynet}\\
                                                         In-house video data\end{tabular} 
                                                                                                             & 17.3     \\ \midrule
Caption                     & \begin{tabular}[c]{@{}c@{}}CC12M \citep{changpinyo2021conceptual}\\
                                                         ShareGPT4V \citep{chen2023sharegpt4v}\\
                                                         VizWiz-Captions \citep{gurari2020captioning}\\
                                                         SBU \citep{ordonez2011im2text}\\
                                                         Flickr30K \citep{young2014image}\\
                                                         Microsoft COCO Captions \citep{chen2015microsoft}\\
                                                         Taisu \citep{liu2022taisu}\\
                                                         ALLaVA-4V \citep{chen2024allava}\\
                                                         Laion-400M \citep{schuhmann2021laion}\\
                                                         CC3M \citep{sharma2018conceptual}\\
                                                         TextCaps \citep{sidorov2020textcaps}\\
                                                         In-house caption data\end{tabular}                   & 9.0      \\ \midrule
Text-only                   & \begin{tabular}[c]{@{}c@{}}RedPajama \citep{together2023redpajama}\\
                                                         Alpaca \citep{taori2023stanford}\\
                                                         Belle \citep{BELLE}\\
                                                         DeepCtrl-sft-data \citep{DeepCtrl-sft-data}\\
                                                         Wudao \citep{Wudao}\\
                                                         Telechat \citep{wang2024telechat}\\
                                                         Firefly \citep{Firefly}\\
                                                         pCLUE \citep{pCLUE}\\
                                                         Guanaco \citep{Guanaco} \end{tabular}                                                                                                                                                                    & 7.7      \\ \midrule
VQA                         & \begin{tabular}[c]{@{}c@{}}VQAv2 \citep{goyal2017making}\\
                                                         M3IT \citep{li2023m}\\
                                                         VizWiz-VQA \citep{gurari2018vizwiz}\\
                                                         OCR-VQA \citep{mishra2019ocr}\\
                                                         VSR \citep{liu2023visual}\\
                                                         OK-VQA \citep{marino2019ok}\\
                                                         VisDial \citep{das2017visual} \\
                                                         A-OKVQA \citep{schwenk2022okvqa}\\
                                                         TextVQA \citep{singh2019towards}\\
                                                         GQA \citep{hudson2019gqa}\\
                                                         In-house VQA data\end{tabular}                            & 7.5      \\ \midrule
Grounding                   & \begin{tabular}[c]{@{}c@{}}GoldG \citep{li2022grounded}\\
                                                         In-house grounding data \end{tabular}                           & 4.1      \\ \midrule
Localization                & \begin{tabular}[c]{@{}c@{}}RefCOCO\\
                                                         RefCOCO+\\
                                                         RefCOCOg \citep{yu2016modeling} \end{tabular}         & 0.5     \\   
\end{longtable}


\begin{longtable}[ht]{@{}ccc@{}}
\caption{\textbf{Summary of datasets used in the multimodal supervised instruction tuning stage}}
\label{Summary_of_sft_stage} \\
\toprule
Category    & Dataset   & Ratio/\% \\ \midrule
\endfirsthead
\caption[]{\textbf{Summary of datasets used in the multimodal supervised instruction tuning stage (Continued)}} \\
\toprule
Category     & Dataset      & Ratio/\% \\ \midrule
\endhead
\bottomrule
\endlastfoot
Multi-images task          & Mantis-Instruct \citep{jiang2024mantis}            & 39.70    \\ \midrule
General VQA                & \begin{tabular}[c]{@{}c@{}}COCO-QA \citep{ren2015exploring}\\
                             Visual7W \citep{zhu2016visual7w}\\
                             VQAv2 \citep{goyal2017making}\\
                             TallyQA \citep{acharya2019tallyqa}\\
                             HatefulMemes \citep{kiela2020hateful}\\
                             VQA-RAD \citep{lau2018dataset}\\
                             LLaVA-Instruct-150K \citep{liu2024improved}\\
                             M3IT \citep{li2023m} \\
                             ALLaVA-Instruct-4V \citep{chen2024allava}
                             \end{tabular}                                       & 36.86    \\ \midrule
Text-only task             & \begin{tabular}[c]{@{}c@{}}OpenHermes-2.5 \citep{OpenHermes_2.5}\\
                             Dolly \citep{conover2023free}\\
                             MetaMathQA \citep{yu2023metamath}\\
                             MathInstruct \citep{yue2023mammoth}\\
                             CamelAIMath \citep{li2023camel}\\
                             AtlasMathSets \citep{AtlasMathSets}\\
                             Goat \citep{liu2023goat}\\
                             CoT \citep{alpaca-cot}\\
                             pCLUE \citep{pCLUE}\\
                             Firefly \citep{Firefly}\\
                             COIG \citep{zhang2023chinese}\\
                             Alpaca \citep{taori2023stanford} \end{tabular}                                  & 11.43    \\ \midrule
Video-related task         & \begin{tabular}[c]{@{}c@{}}Video Instruction \citep{Maaz2023VideoChatGPT}\\
                             InternVideo \citep{wang2022internvideo}\\
                             Video-ChatGPT-100K \citep{Maaz2023VideoChatGPT} \end{tabular}                   & 5.31     \\ \midrule
Chart/figure understanding & \begin{tabular}[c]{@{}c@{}}Chart2Text \citep{Maaz2023VideoChatGPT}\\
                             DVQA \citep{kafle2018dvqa}\\
                             ChartQA \citep{masry2022chartqa}\\
                             FigureQA \citep{kahou2017figureqa}\\
                             MapQA \citep{chang2022mapqa} \\
                             MMC-Instruction \citep{liu2023mmc} \end{tabular}                                & 2.18     \\ \midrule
OCR-related task           & \begin{tabular}[c]{@{}c@{}}RenderedText \citep{RenderedText}\\
                             DocVQA \citep{mathew2021docvqa}\\
                             TextVQA \citep{singh2019towards}\\
                             ST-VQA \citep{biten2019scene}\\
                             VisualMRC \citep{tanaka2021visualmrc}\\
                             IAM \citep{marti2002iam}\\
                             InfoVQA \citep{mathew2022infographicvqa}\\
                             Diagram image-to-text \citep{image-to-text}\\
                             RCTW-17 \citep{shi2017icdar2017} \\
                             ReCTS \citep{yao2012detecting} \end{tabular}                                   & 1.64     \\ \midrule
Table understanding        & \begin{tabular}[c]{@{}c@{}}TabMWP \citep{lu2022dynamic}\\
                             TAT-QA \citep{zhu2021tat}\\
                             HiTab \citep{cheng2021hitab}\\
                             MultiHiertt \citep{zhao2022multihiertt}\\
                             FinQA \citep{chen2021finqa}\\
                             WikiSQL \citep{zhong2017seq2sql}\\
                             SQA \citep{iyyer2017search}\\
                             WTQ \citep{pasupat2015compositional} \end{tabular}                             & 1.10     \\ \midrule
Logical reasoning and Math & \begin{tabular}[c]{@{}c@{}}GeomVerse \citep{kazemi2023geomverse}\\
                             CLEVR-Math \citep{lindstrom2022clevr}\\
                             CLEVR \citep{johnson2017clevr}\\
                             IconQA \citep{lu2021iconqa}\\
                             RAVEN \citep{zhang2019raven}\\
                             Inter-GPs \citep{lu2021inter} \end{tabular}                                    & 0.86     \\ \midrule
Image Captioning           & \begin{tabular}[c]{@{}c@{}}LNarratives \citep{pont2020connecting}\\
                             Screen2Words \citep{wang2021screen2words}\\
                             ShareGPT4V \citep{chen2023sharegpt4v} \\
                             In-house caption data
                             \end{tabular}                                        & 0.55     \\ \midrule
Image comparison           & \begin{tabular}[c]{@{}c@{}}NLVR2 \citep{suhr2018corpus}\\
                             GSD \citep{li2023mimic}\\
                             Spot the diff \citep{jhamtani2018learning} \end{tabular}                       & 0.22     \\ \midrule
Knowledge QA               & \begin{tabular}[c]{@{}c@{}}AI2D \citep{kembhavi2016diagram}\\
                             TQA \citep{kembhavi2017you}\\
                             ScienceQA \citep{lu2022learn} \end{tabular}                                    & 0.14     \\ \midrule
Code generation            & \begin{tabular}[c]{@{}c@{}}WebSight \citep{laurenccon2024unlocking}\\
                             DaTikz \citep{belouadi2023automatikz} \end{tabular}                            & 0.03    
\end{longtable}


\begin{figure}[htbp]
  \centering  \includegraphics[width=14.5cm, height=21cm]{show_case_v11_2.png}
  \caption{\textbf{Examples of OmChat Handling Various Tasks}}
  \label{show1}
\end{figure}

\begin{figure}[htbp]
  \centering  \includegraphics[width=14.5cm, height=21cm]{show_case_v11_1.png}
  \caption{\textbf{More Examples of OmChat Handling Various Tasks}}
  \label{show2}
\end{figure}
